Fast, Fair and Truthful Distributed Stable Matching for Common Preferences

Stable matching is a fundamental problem studied both in economics and computer science. The task is to find a matching between two sides of agents that have preferences over who they want to be matched with. A matching is stable if no pair of agents prefer each other over their current matches. The deferred acceptance algorithm of Gale and Shapley solves this problem in polynomial time. Further, it is a mechanism: the proposing side in the algorithm is always incentivised to report their preferences truthfully. The deferred acceptance algorithm has a natural interpretation as a distributed algorithm (and thus a distributed mechanism). However, the algorithm is slow in the worst case and it is known that the stable matching problem cannot be solved efficiently in the distributed setting. In this work we study a natural special case of the stable matching problem where all agents on one side share common preferences. We show that in this case the deferred acceptance algorithm does yield a fast and truthful distributed mechanism for finding a stable matching. We show how algorithms for sampling random colorings can be used to break ties fairly and extend the results to fractional stable matching.

==> related-work.tex <==
% !TEX root = sample-acmsmall-submission.tex
%\subsection{Related work}


%any fast truthful mechanism has doen before? distributed or centralized
%Gale and Shapley (DA)
In their pioneering work, Gale and Shapley \cite{gale62sm} addressed the matching problem in the following setting: consider two sets of agents, containing $n$ men and $m$ women, where each agent individually ranks all members of the opposite gender. The objective is to form a matching, a one-to-one correspondence between agents, that is stable, meaning it is free from blocking pairs where agents mutually prefer each other over their assigned partners in the matching. Gale and Shapley proved the existence of a stable matching. The centralized Gale-Shapley algorithm has a time complexity of ($O(n^2)$), which is reasonable for centralized algorithms. Knuth \cite{knuth1997stable} provided a comprehensive review of stable marriage problem. 

Recently there are several works in the literature focusing on  approximate versions of the stable marriage problem, specially in distributed setting \cite{floreen10stable, AbrahamAlmost, eriksson2008instability, hassidim2016local} , the goal of this works are finding the matching which is almost stable. the authors in \cite{eriksson2008instability} claim that the  best measure of instability is the  proportion of blocking pairs among all possible pairs. 


Hassidim, Mansour, and Vardi \cite{hassidim2016local} formalize the notion of local computation mechanism design for stable matching, job scheduling, and combinatorial auctions. They showed that for bounded preference lists, terminating the Gale-Shapley algorithm after a fixed number of iterations results in a good approximation to the stable matching. More recently, Ostrovsky and Rosenbaum \cite{ostrovsky2015fast} obtained similar results, considering an approximate version of the stable marriage problem where an almost stable matching induces $\epsilon |M|$ blocking pairs, where $|M|$ is the size of the produced matching. {\AA}strand and Suomela \cite{Astrand2010} investigate maximal edge packing in a weighted graph within a distributed setting. They demonstrate that regardless of the number of nodes in the network, achieving maximal edge packing is possible in $O(\Delta + \log^* W)$ , where $\Delta$ represents the maximum degree of the graph and $W$ denotes the maximum weight.

FIXME: Khanchandani and Wattenhofer~\cite{khanchandani16distributed}
FIXME: Kipnis and Patt-Shamir~\cite{Kipnis09note}


Flor{\'{e}}en, Kaski, Polishchuk, and Suomela \cite{floreen10stable}, also study the  local version of Gale–Shapley algorithm  for the stable marriage problem. They  aim at finding a matching with few unstable edges. The results show for bounded preference lists, truncating the Gale-Shapley algorithm after some  communications rounds yields a matching with  a constant ratio of unstable edges to matching edges.
%In \cite{floreen10stable}, the authors examine the local version of the Gale–Shapley algorithm \cite{gale62sm} for the stable marriage problem. They demonstrate that the number of matched agents has a linear proportion to the number of executed rounds by the Gale–Shapley algorithm.
This leads to an important consequence: agents can achieve an almost stable matching with just local information about their neighbors, without requiring full information about the entire network. This can have a significant impact, especially in large distributed networks.

The main idea in this paper lies in the analysis of the "transient phase" of the Gale–Shapley algorithm by truncating the algorithm to a specific number of rounds. They show that with a constant number of rounds, only a few unstable edges (constant ratio) are obtained compared to the matching edges. This work is particularly close to ours, however, terminating the algorithm after some rounds raises issues of untruthfulness.


%FIXME: 
Ostrovsky and Rosenbaum \cite{ostrovsky2015fast} present a new deterministic distributed algorithm which finds an almost stable matching faster than \cite{floreen10stable} they achieve $O(\log^5n)$  an arbitrary in a randomized variant which requires $O(\log^2 n)$  rounds. However they also didn't consider the incentive compatibility for the proposed solution. 




%Distributed algorithmic mechanism design



Distributed Algorithmic Mechanism Design (DAMD) merges the traditional emphasis of theoretical computer science on computational feasibility with its newer attention to incentive compatibility and distributed computing \cite{borgers2015introduction}.
Game theory explores the outcomes when rational agents act in their own self-interest. Mechanism design, on the other hand, delves into designing systems in a way that encourages agents to achieve desired system  goals. The "mechanisms" in this context refer to the specifications of outcomes and payments to agents, which incentivise them to act in a manner that aligns with the desired overall outcome.

 Feigenbaum and Shenker \cite{FeigenbaumS03} provide an in-depth overview of Distributed Algorithmic Mechanism Design (DAMD), covering its technical foundations, the role of approximations, and strategic models. They review DAMD results on multicast cost-sharing and interdomain routing, and they identify several promising areas for future research.

Afek and Ginzberg \cite{AfekGFS13} generalize the game-theoretic model of distributed computing. Building upon the work by Abraham, Dolev, and Halpern \cite{AbrahamDH19}, they offer resilient protocols for basic building blocks like knowledge sharing and wake-up, and utilize them to obtain protocols for consensus, renaming, and leader election. These protocols operate under assumptions about agents’ preferences, including an agent having a strict preference for outcomes in which it learns the input of other agents.
% they  take into account the factors that might affect the utilities of agents in a distributed setting, and the actions that they may take as a result of these factors
%provide protocols for consensus with crash failures and rational agents




%%% Stable matching in CS: support for the model: School choice, cashing, edge computing, economic
% mention the case for same provides. 

Matching mechanisms are frequently employed in the design and functioning of both industrial and academic communities, as well as real-world markets. Examples of such applications include student housing \cite{chen2002improving}, central kidney exchange design \cite{roth2004kidney}, and school choice systems (\cite{abdulkadirouglu2003school, Pathakschoolchoice}.%add some references

%Particularly, the Deferred Acceptance (DA) algorithm, which is considered in this work, is utilized by numerous school districts across Europe and the US for assigning students to public schools and graduates to university positions.

Here, we delve into specific scenarios where matching algorithms are employed:
School choice is one of the widely discussed topics in education, where students have the opportunity to choose the school they will attend. Traditionally, students are assigned to public schools based on their residential location, which is considered unfair. In this problem, there are a number of students, each of whom should be assigned a seat at one of a number of schools. Each school has a maximum capacity, but the total number of seats is sufficient. Each student has strict preferences over all schools, and each school has a strict priority ordering of all students \cite{abdulkadirouglu2003school}

%In school choice, the main issue is the design of a student assignment mechanism.
The school choice problem is closely related to the well-known college admissions problem introduced by Gale and Shapley. The key difference between the two problems is that in school choice, schools are objects to be "consumed" by the students, whereas in college admissions, schools themselves are agents who have preferences over students. The outcome of a school choice problem is an assignment of schools to students such that each student is assigned one school and no school is assigned to more students than its capacity \cite{NBERw11965}.
%FIXME: do we need more detail here?

%Gale-Shapley student optimal stable mechanism has one additional very appealing feature: It is strategy-proof. That is, truthful preference revelation is a dominant strategy for the stu- dents. In particular, students and their parents do not need to worry about losing their priorities as a consequence of reporting their truthful preferences. Gale-Shapley student optimal stable mechanism relieves students and their parents of devising complicated admissions strategies.


%Introduction about IoT, then cloud, then edge and cooperative computing, 

The Internet of Things (IoT) encompasses a large number of uniquely addressable smart devices and supports diverse applications, interacting in non-trivial ways \cite{ATZORI20102787}.
%This vision foresees billions of everyday physical objects, equipped with different capabilities, to be connected to the Internet and enhanced with intelligence to make our environment smart.
%Such networks are increasingly used for edge analytics, i.e., collecting and analyzing data at the network edge.
\begin{comment}
However, IoT devices are typically resource-constrained and cannot support fast and accurate execution of such tasks, while the involvement of distant cloud servers is often impractical and entails huge communication overheads \cite{Farris2017}. 
%Fog computing \cite{FogComputing} has emerged to address the issues of Cloud-based solutions,
%A recent popular approach is to move micro data centers towards the edge of the network, Mobile Edge Computing (MEC),Fog Computing  .
%Moving forward on this road, several substantial works have emerged in literature around the 
 Recently, opportunistic cooperation among IoT devices has emerged to address the issues of Cloud-based solutions\cite{Farris2017,RanjbaranAuction,RanjbaranSocialMatching}.
%for the creation of dynamic local clouds 

The idea of finding the best match to offload the tasks of IoT devices at the edge  has received a lot of attention in recent years.
 %There is a lot of works in the literature that models offloading as a matching problem, 
 Where  IoT devices are on one side and micro-data centers on the other side of the network. For example, 
 %Liu, Li and Sun \cite{VehicularPengju} proposed a matching-based task offloading algorithm is considered in vehicular IoT networks to minimize network delay, involving both one-to-one and one-to-many matching. 
 Ranjbaran, Nitti and Manshaei \cite{RanjbaranSocialMatching} developed a Many-to-Many (M-M) assignment game based on matching theory is used to support cooperation among devices to share their resources and create ad hoc local clouds.
\end{comment}

However, IoT devices are typically resource-constrained and cannot support fast and accurate task execution. Involvement of distant cloud servers is often impractical and entails significant communication overheads \cite{Farris2017}.

Recently, opportunistic cooperation among IoT devices has emerged to address issues with Cloud-based solutions \cite{Farris2017, RanjbaranAuction, RanjbaranSocialMatching}.

The idea of finding the best match to offload tasks from IoT devices at the edge has garnered significant attention in recent years. For instance, Ranjbaran, Nitti, and Manshaei \cite{RanjbaranSocialMatching} developed a Many-to-Many (M-M) assignment game based on matching theory to support cooperation among devices, facilitating resource sharing and the creation of ad hoc local clouds.  Liu, Li and Sun \cite{VehicularPengju} proposed a matching-based task offloading algorithm is considered in vehicular IoT networks to minimize network delay, involving both one-to-one and one-to-many matching.

%FIXME should I go to more details or specify the difference with this work?
%%%%%%%%%%%%%%%%%%% specific Scenario the practical point of view
Our proposed solution can serve as an efficient and reliable method for addressing such problems. The assumption of identical providers and common preferences aligns perfectly with the edge offloading problem, where providers can be likened to data centers or IoT devices with spare resources without customized preferences over IoT users. 

\begin{comment}
Here, we explore a specific scenario in the IoT domain where our algorithm can be applied in a practical context:
Consider cooperative task sharing in  Mobile Edge Learning (MEL) era. Where,there is a high variability in computation (i.e., in CPU and memory workload) as well as the task properties among IoT devices. 
We propose a framework based on matching theory in order to find the best possible node to outsource the task. 
In this setting lets consider a compact smart city neighborhood that houses a wireless Internet of Things (IoT) network consisting of various types of devices and a single gateway known as the Edge Provider (EP). This network features heterogeneous devices that generate different learning tasks over time, such as face recognition in smart doorbells or object detection in traffic management cameras. 

If each device had enough resources (computation, energy) and accurately-enough inference libraries for the tasks that it receives, then the devices could operate in a stand-alone fashion. However, more often than not, this is not the case. For example, a robot might have a Neural Network (NN) that is exceptionally-well trained to detect animals in video frames, but performs poorly when it comes to detection of vehicles. Similarly, a node might have ample computing capacity (e.g., a high-performing GPU), but at a given moment suffer from low energy availability. On the other hand there are some devices with spare resources which can be the host for the neighboring devices.

The devices in this network are interconnected by links of varying capacity and allocate their energy resources for data exchange and/or local task computation. Our objective  is to develop cooperative task execution policies in such IoT networks, aiming to leverage the inherent complementary of resources, requirements and capabilities of the nodes, towards maximizing an aggregate network-wide performance-cost metric.
%In their pioneering work, Gale and Shapley addressed the matching problem in the following setting: consider two sets of agents, containing $n$ men and $m$ women, where each agent individually ranks all members of the opposite gender. The objective is to form a matching, a one-to-one correspondence between agents, that is stable, meaning it is free from blocking pairs where agents mutually prefer each other over their assigned partners in the matching. Gale and Shapley proved the existence of a stable matching. The centralized Gale-Shapley algorithm has a time complexity of ($O(n^2)$), which is reasonable for centralized algorithms. In \cite{knuth1997stable},  a comprhenive review of stable marriage problem is provided. 
\end{comment}
%Examples for matching in realworld setting: 
%%%%SARA FIXME Matching algorithms are  frequently used in real-world markets. Examples include school selection, organizing kidney exchanges for patients. edge commputing and cashing, are the examples of 

